PathoGaze1.0: An AI-Ready Navigation, Eye-Tracking, and Decision Dataset in Pathology

Performing cancer diagnosis on giga-pixel whole-slide images (WSIs) is an important but difficult visual search task. The large giga-pixel image size forces pathologists to navigate by zooming and panning to search tissue for malignancy. Diagnostic accuracy averages around 70%, and adding a second pathologist does not substantially improve consistencies between diagnoses. There is a lack of publicly available behavioral data to explain these diagnostic errors and inconsistencies. To fill this gap, we curated PathoGaze1.0, a comprehensive behavioral dataset capturing high-fidelity clinical diagnostic workflows across 11 different pathologist participants over two experiments 12-months apart (8 overlapping pathologists across both experiments), as they interpreted 397 WSIs from CAMELYON16, a set of publicly available breast cancer lymph node WSIs. The dataset comprises 18.69 hours of eye-tracking (171,909 fixations), and navigational scanning data along with 1,140 diagnostic decisions, all collected using a newly-developed testbed PTAH. The testbed supports interaction techniques found in clinical tools and collects viewport, mouse actions, and diagnostic decisions, enabling cross-links between WSI image stimulus, gaze, navigation behaviors, and diagnostic decisions. We share preregistered experimental materials, the datasets, and processing methods on the Open Science Framework (OSF).

==> bibliography.tex <==
\begin{thebibliography}{10}
\urlstyle{rm}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\expandafter\ifx\csname doiprefix\endcsname\relax\def\doiprefix{DOI: }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{balogh2015improving}
\bibinfo{author}{Balogh, E.~P.}, \bibinfo{author}{Miller, B.~T.} \& \bibinfo{author}{Ball, J.~R.}
\newblock \emph{\bibinfo{title}{Improving diagnosis in health care}} (\bibinfo{publisher}{National Academies Press (US)}, \bibinfo{year}{2015}).

\bibitem{west2018physician}
\bibinfo{author}{West, C.~P.}, \bibinfo{author}{Dyrbye, L.~N.} \& \bibinfo{author}{Shanafelt, T.~D.}
\newblock \bibinfo{journal}{\bibinfo{title}{Physician burnout: contributors, consequences and solutions}}.
\newblock {\emph{\JournalTitle{J. Intern. Med.}}} \textbf{\bibinfo{volume}{283}}, \bibinfo{pages}{516--529}, \href{https://doi.org/10/ggcsdv}{10/ggcsdv} (\bibinfo{year}{2018}).

\bibitem{drew2021more}
\bibinfo{author}{Drew, T.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{More scanning, but not zooming, is associated with diagnostic accuracy in evaluating digital breast pathology slides}}.
\newblock {\emph{\JournalTitle{J. Vision}}} \textbf{\bibinfo{volume}{21}}, \bibinfo{pages}{1--17}, \href{https://doi.org/10/pz48}{10/pz48} (\bibinfo{year}{2021}).

\bibitem{molin2015slide}
\bibinfo{author}{Molin, J.}, \bibinfo{author}{Fjeld, M.}, \bibinfo{author}{Mello-Thoms, C.} \& \bibinfo{author}{Lundstr{\"o}m, C.}
\newblock \bibinfo{journal}{\bibinfo{title}{Slide navigation patterns among pathologists with long experience of digital review}}.
\newblock {\emph{\JournalTitle{Histopathology}}} \textbf{\bibinfo{volume}{67}}, \bibinfo{pages}{185--192} (\bibinfo{year}{2015}).

\bibitem{parwani2021whole}
\bibinfo{author}{Parwani, A.~V.}
\newblock \emph{\bibinfo{title}{Whole Slide Imaging: Current Applications and Future Directions}} (\bibinfo{publisher}{Springer}, \bibinfo{year}{2021}).

\bibitem{forlines2009improving}
\bibinfo{author}{Forlines, C.} \& \bibinfo{author}{Balakrishnan, R.}
\newblock \bibinfo{title}{Improving visual search with image segmentation}.
\newblock In \emph{\bibinfo{booktitle}{Proc. SIGCHI.}}, \bibinfo{pages}{1093--1102}, \href{https://doi.org/10/ftqgsc}{10/ftqgsc} (\bibinfo{year}{2009}).

\bibitem{plumlee2006zooming}
\bibinfo{author}{Plumlee, M.~D.} \& \bibinfo{author}{Ware, C.}
\newblock \bibinfo{journal}{\bibinfo{title}{Zooming versus multiple window interfaces: Cognitive costs of visual comparisons}}.
\newblock {\emph{\JournalTitle{ACM Transactions on Computer-Human Interaction (TOCHI)}}} \textbf{\bibinfo{volume}{13}}, \bibinfo{pages}{179--209} (\bibinfo{year}{2006}).

\bibitem{kockwelp199martha}
\bibinfo{author}{Kockwelp, J.}, \bibinfo{author}{Kliesch, S.}, \bibinfo{author}{Gromoll, J.}, \bibinfo{author}{Wistuba, J.} \& \bibinfo{author}{Risse, B.}
\newblock \bibinfo{journal}{\bibinfo{title}{{MARTHA-Combining gaze into deep learning for fully quantitative human testicular histology analysis}}}.
\newblock {\emph{\JournalTitle{Comput. Biol. Med.}}} \textbf{\bibinfo{volume}{199}}, \bibinfo{pages}{111270}, \href{https://doi.org/10/rhv8}{10/rhv8} (\bibinfo{year}{2026}).

\bibitem{lopes2026exploring}
\bibinfo{author}{Lopes, A.}, \bibinfo{author}{Chin-Yee, B.}, \bibinfo{author}{Wang, L.}, \bibinfo{author}{Cecchini, M.~J.} \& \bibinfo{author}{Ward, A.~D.}
\newblock \bibinfo{title}{Exploring fixational eye movements for mitotic figure differentiation in digital pathology}.
\newblock In \emph{\bibinfo{booktitle}{Proc. Med. Imaging}}, vol. \bibinfo{volume}{13932}, \bibinfo{pages}{179--189}, \href{https://doi.org/10/rhw2}{10/rhw2} (\bibinfo{organization}{SPIE}, \bibinfo{year}{2026}).

\bibitem{sprinkle2024comparing}
\bibinfo{author}{Sprinkle, S.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Comparing viewing skills of digital images among cytologists, pathology residents and experienced pathologists using eye tracking technology}}.
\newblock {\emph{\JournalTitle{J. Am. Soc. Cytopathol.}}} \textbf{\bibinfo{volume}{13}}, \bibinfo{pages}{S10}, \href{https://doi.org/10/rhw3}{10/rhw3} (\bibinfo{year}{2024}).

\bibitem{nan2025deep}
\bibinfo{author}{Nan, T.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Deep learning quantifies pathologists’ visual patterns for whole slide image diagnosis}}.
\newblock {\emph{\JournalTitle{Nat. Commun.}}} \textbf{\bibinfo{volume}{16}}, \bibinfo{pages}{5493}, \href{https://doi.org/10/p274}{10/p274} (\bibinfo{year}{2025}).

\bibitem{drew2023pathologist}
\bibinfo{author}{Drew, T.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Pathologist pupil dilation reflects experience level and difficulty in diagnosing medical images}}.
\newblock {\emph{\JournalTitle{J. Med. Imaging}}} \textbf{\bibinfo{volume}{10}}, \bibinfo{pages}{025503--025503}, \href{https://doi.org/10/q5kw}{10/q5kw} (\bibinfo{year}{2023}).

\bibitem{brunye2023image}
\bibinfo{author}{Bruny{\'e}, T.~T.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{From image to diagnosis: characterizing sources of error in histopathologic interpretation}}.
\newblock {\emph{\JournalTitle{Mod. Pathol.}}} \textbf{\bibinfo{volume}{36}}, \bibinfo{pages}{100162}, \href{https://doi.org/10/pz5b}{10/pz5b} (\bibinfo{year}{2023}).

\bibitem{brunye2023zoom}
\bibinfo{author}{Bruny{\'e}, T.~T.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Zoom behavior during visual search modulates pupil diameter and reflects adaptive control states}}.
\newblock {\emph{\JournalTitle{{PLoS One}}}} \textbf{\bibinfo{volume}{18}}, \bibinfo{pages}{e0282616}, \href{https://doi.org/10/rf4r}{10/rf4r} (\bibinfo{year}{2023}).

\bibitem{mariam2022smart}
\bibinfo{author}{Mariam, K.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{On smart gaze based annotation of histopathology images for training of deep convolutional neural networks}}.
\newblock {\emph{\JournalTitle{J. Biomed. Health. Inf.}}} \textbf{\bibinfo{volume}{26}}, \bibinfo{pages}{3025--3036}, \href{https://doi.org/10/g5p2n4}{10/g5p2n4} (\bibinfo{year}{2022}).

\bibitem{sudin2021eye}
\bibinfo{author}{Sudin, E.} \emph{et~al.}
\newblock \bibinfo{title}{Eye tracking in digital pathology: identifying expert and novice patterns in visual search behaviour}.
\newblock In \emph{\bibinfo{booktitle}{Medical Imaging 2021: Digital Pathology}}, vol. \bibinfo{volume}{11603}, \bibinfo{pages}{253--262}, \href{https://doi.org/10/rtgt}{10/rtgt} (\bibinfo{organization}{SPIE}, \bibinfo{year}{2021}).

\bibitem{kimeswenger2021artificial}
\bibinfo{author}{Kimeswenger, S.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Artificial neural networks and pathologists recognize basal cell carcinomas based on different histological patterns}}.
\newblock {\emph{\JournalTitle{Modern Pathology}}} \textbf{\bibinfo{volume}{34}}, \bibinfo{pages}{895--903}, \href{https://doi.org/10/rtgs}{10/rtgs} (\bibinfo{year}{2021}).

\bibitem{brunye2017accuracy}
\bibinfo{author}{Bruny{\'e}, T.~T.}, \bibinfo{author}{Mercan, E.}, \bibinfo{author}{Weaver, D.~L.} \& \bibinfo{author}{Elmore, J.~G.}
\newblock \bibinfo{journal}{\bibinfo{title}{Accuracy is in the eyes of the pathologist: the visual interpretive process and diagnostic accuracy with digital whole slide images}}.
\newblock {\emph{\JournalTitle{J. Biomed. Inf.}}} \textbf{\bibinfo{volume}{66}}, \bibinfo{pages}{171--179}, \href{https://doi.org/10/gfxsg9}{10/gfxsg9} (\bibinfo{year}{2017}).

\bibitem{Chakraborty}
\bibinfo{author}{Chakraborty, S.} \emph{et~al.}
\newblock \bibinfo{title}{{Visual Attention Analysis Of Pathologists Examining Whole Slide Images Of Prostate Cancer}}.
\newblock In \emph{\bibinfo{booktitle}{IEEE International Symposium on Biomedical Imaging}}, \bibinfo{pages}{1--5}, \href{https://doi.org/10/rt9q}{10/rt9q} (\bibinfo{year}{2022}).

\bibitem{lopes2024eye}
\bibinfo{author}{Lopes, A.}, \bibinfo{author}{Ward, A.~D.} \& \bibinfo{author}{Cecchini, M.}
\newblock \bibinfo{journal}{\bibinfo{title}{Eye tracking in digital pathology: a comprehensive literature review}}.
\newblock {\emph{\JournalTitle{J. Pathol. Inf.}}} \textbf{\bibinfo{volume}{15}}, \bibinfo{pages}{100383}, \href{https://doi.org/10/gvm7zt}{10/gvm7zt} (\bibinfo{year}{2024}).

\bibitem{akhtar2024croissant}
\bibinfo{author}{Akhtar, M.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Croissant: A metadata format for ml-ready datasets}}.
\newblock {\emph{\JournalTitle{Advances in Neural Information Processing Systems}}} \textbf{\bibinfo{volume}{37}}, \bibinfo{pages}{82133--82148} (\bibinfo{year}{2024}).

\bibitem{osfdataset}
\bibinfo{author}{Thai, V.} \emph{et~al.}
\newblock \bibinfo{title}{{PathoGaze1.0: An AI-Ready Navigation Tracking Eye-Tracking, and Decision Dataset in Pathology}}, \href{https://doi.org/10.17605/OSF.IO/HJ9A7}{10.17605/OSF.IO/HJ9A7} (\bibinfo{year}{2026}).

\bibitem{bejnordi2017diagnostic}
\bibinfo{author}{Bejnordi, B.~E.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Diagnostic assessment of deep learning algorithms for detection of lymph node metastases in women with breast cancer}}.
\newblock {\emph{\JournalTitle{J. Am. Med. Assoc.}}} \textbf{\bibinfo{volume}{318}}, \bibinfo{pages}{2199--2210}, \href{https://doi.org/10/gcn2kf}{10/gcn2kf} (\bibinfo{year}{2017}).

\bibitem{nuthmann2021effect}
\bibinfo{author}{Nuthmann, A.}, \bibinfo{author}{Clayden, A.~C.} \& \bibinfo{author}{Fisher, R.~B.}
\newblock \bibinfo{journal}{\bibinfo{title}{The effect of target salience and size in visual search within naturalistic scenes under degraded vision}}.
\newblock {\emph{\JournalTitle{J. Vision}}} \textbf{\bibinfo{volume}{21}}, \bibinfo{pages}{2--2}, \href{https://doi.org/10/rt9p}{10/rt9p} (\bibinfo{year}{2021}).

\bibitem{CAMELYON17}
\bibinfo{author}{Litjens, G.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{{1399 H\&E-stained sentinel lymph node sections of breast cancer patients: the CAMELYON dataset}}}.
\newblock {\emph{\JournalTitle{GigaScience}}} \textbf{\bibinfo{volume}{7}}, \href{https://doi.org/10.1093/gigascience/giy065}{10.1093/gigascience/giy065} (\bibinfo{year}{2018}).

\bibitem{budginaite2024computational}
\bibinfo{author}{Budginaite, E.}, \bibinfo{author}{Magee, D.~R.}, \bibinfo{author}{Kloft, M.}, \bibinfo{author}{Woodruff, H.~C.} \& \bibinfo{author}{Grabsch, H.~I.}
\newblock \bibinfo{journal}{\bibinfo{title}{Computational methods for metastasis detection in lymph nodes and characterization of the metastasis-free lymph node microarchitecture: A systematic-narrative hybrid review}}.
\newblock {\emph{\JournalTitle{J. Pathol. Inf.}}} \textbf{\bibinfo{volume}{15}}, \bibinfo{pages}{100367}, \href{https://doi.org/10/pz4n}{10/pz4n} (\bibinfo{year}{2024}).

\bibitem{leube2017sampling}
\bibinfo{author}{Leube, A.}, \bibinfo{author}{Rifai, K.} \& \bibinfo{author}{Wahl, S.}
\newblock \bibinfo{journal}{\bibinfo{title}{Sampling rate influences saccade detection in mobile eye tracking of a reading task}}.
\newblock {\emph{\JournalTitle{J. Eye Mov. Res.}}} \textbf{\bibinfo{volume}{10}}, \bibinfo{pages}{16} (\bibinfo{year}{2017}).

\bibitem{OpenSeadragon}
\bibinfo{author}{{OpenSeadragon contributors}}.
\newblock \bibinfo{title}{{OpenSeadragon}}.
\newblock \bibinfo{howpublished}{https://openseadragon.github.io/} (\bibinfo{year}{2022}).
\newblock \bibinfo{note}{Version 3.1.0}.

\bibitem{Annotorious}
\bibinfo{author}{{Annotorious contributors}}.
\newblock \bibinfo{title}{{Annotorious}}.
\newblock \bibinfo{howpublished}{https://annotorious.github.io/} (\bibinfo{year}{2022}).

\bibitem{olsen2012tobii}
\bibinfo{author}{Olsen, A.}
\newblock \bibinfo{title}{{The Tobii I-VT fixation filter}}.
\newblock \bibinfo{howpublished}{https://go.tobii.com/Tobii-I-VT-fixation-filter-white-paper} (\bibinfo{year}{2012}).

\bibitem{gisev2013interrater}
\bibinfo{author}{Gisev, N.}, \bibinfo{author}{Bell, J.~S.} \& \bibinfo{author}{Chen, T.~F.}
\newblock \bibinfo{journal}{\bibinfo{title}{Interrater agreement and interrater reliability: key concepts, approaches, and applications}}.
\newblock {\emph{\JournalTitle{Research in Social and Administrative Pharmacy}}} \textbf{\bibinfo{volume}{9}}, \bibinfo{pages}{330--338} (\bibinfo{year}{2013}).

\bibitem{krippendorff2004reliability}
\bibinfo{author}{Krippendorff, K.}
\newblock \bibinfo{journal}{\bibinfo{title}{Reliability in content analysis: Some common misconceptions and recommendations}}.
\newblock {\emph{\JournalTitle{Human Communication Research}}} \textbf{\bibinfo{volume}{30}}, \bibinfo{pages}{411--433}, \href{https://doi.org/10.1111/j.1468-2958.2004.tb00738.x}{10.1111/j.1468-2958.2004.tb00738.x} (\bibinfo{year}{2004}).

\bibitem{gallas2007binary}
\bibinfo{author}{Gallas, B.~D.}, \bibinfo{author}{Pennello, G.~A.} \& \bibinfo{author}{Myers, K.~J.}
\newblock \bibinfo{journal}{\bibinfo{title}{Multireader multicase variance analysis for binary data}}.
\newblock {\emph{\JournalTitle{Journal of the Optical Society of America A}}} \textbf{\bibinfo{volume}{24}}, \bibinfo{pages}{B70--B80}, \href{https://doi.org/10.1364/JOSAA.24.000B70}{10.1364/JOSAA.24.000B70} (\bibinfo{year}{2007}).

\bibitem{Carmody}
\bibinfo{author}{Carmody, D.~P.}, \bibinfo{author}{Nodine, C.~F.} \& \bibinfo{author}{Kundel, H.~L.}
\newblock \bibinfo{journal}{\bibinfo{title}{{An Analysis of Perceptual and Cognitive Factors in Radiographic Interpretation}}}.
\newblock {\emph{\JournalTitle{Perception}}} \textbf{\bibinfo{volume}{9}}, \bibinfo{pages}{339--344}, \href{https://doi.org/10.1068/p090339}{10.1068/p090339} (\bibinfo{year}{1980}).

\bibitem{otsu1975threshold}
\bibinfo{author}{Otsu, N.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{A threshold selection method from gray-level histograms}}.
\newblock {\emph{\JournalTitle{Automatica}}} \textbf{\bibinfo{volume}{11}}, \bibinfo{pages}{23--27}, \href{https://doi.org/10/bfq5pv}{10/bfq5pv} (\bibinfo{year}{1975}).

\bibitem{wu2022functional}
\bibinfo{author}{Wu, C.-C.} \& \bibinfo{author}{Wolfe, J.~M.}
\newblock \bibinfo{journal}{\bibinfo{title}{The functional visual field (s) in simple visual search}}.
\newblock {\emph{\JournalTitle{Vision Res.}}} \textbf{\bibinfo{volume}{190}}, \bibinfo{pages}{107965}, \href{https://doi.org/10/gnvwg2}{10/gnvwg2} (\bibinfo{year}{2022}).

\bibitem{vater2022peripheral}
\bibinfo{author}{Vater, C.}, \bibinfo{author}{Wolfe, B.} \& \bibinfo{author}{Rosenholtz, R.}
\newblock \bibinfo{journal}{\bibinfo{title}{Peripheral vision in real-world tasks: A systematic review}}.
\newblock {\emph{\JournalTitle{Psychonomic Bull. Rev.}}} \textbf{\bibinfo{volume}{29}}, \bibinfo{pages}{1531--1557}, \href{https://doi.org/10/gs3jjx}{10/gs3jjx} (\bibinfo{year}{2022}).

\bibitem{poole2006eye}
\bibinfo{author}{Poole, A.} \& \bibinfo{author}{Ball, L.~J.}
\newblock \bibinfo{title}{{Eye tracking in HCI and usability research}}.
\newblock In \emph{\bibinfo{booktitle}{{Encyclopedia of Human Computer Interaction}}}, \bibinfo{pages}{211--219} (\bibinfo{publisher}{IGI Global Scientific Publishing}, \bibinfo{year}{2006}).

\bibitem{liu2022assessing}
\bibinfo{author}{Liu, J.-C.}, \bibinfo{author}{Li, K.-A.}, \bibinfo{author}{Yeh, S.-L.} \& \bibinfo{author}{Chien, S.-Y.}
\newblock \bibinfo{journal}{\bibinfo{title}{Assessing perceptual load and cognitive load by fixation-related information of eye movements}}.
\newblock {\emph{\JournalTitle{Sensors}}} \textbf{\bibinfo{volume}{22}}, \bibinfo{pages}{1187}, \href{https://doi.org/10/g93q3s}{10/g93q3s} (\bibinfo{year}{2022}).

\bibitem{bylinskii2015eye}
\bibinfo{author}{Bylinskii, Z.}, \bibinfo{author}{Borkin, M.~A.}, \bibinfo{author}{Kim, N.~W.}, \bibinfo{author}{Pfister, H.} \& \bibinfo{author}{Oliva, A.}
\newblock \bibinfo{title}{Eye fixation metrics for large scale evaluation and comparison of information visualizations}.
\newblock In \emph{\bibinfo{booktitle}{ETVIS}}, \bibinfo{pages}{235--255}, \href{https://doi.org/10/q6tz}{10/q6tz} (\bibinfo{organization}{Springer}, \bibinfo{year}{2015}).

\bibitem{mathot2018safe}
\bibinfo{author}{Math{\^o}t, S.}, \bibinfo{author}{Fabius, J.}, \bibinfo{author}{Van~Heusden, E.} \& \bibinfo{author}{Van~der Stigchel, S.}
\newblock \bibinfo{journal}{\bibinfo{title}{Safe and sensible preprocessing and baseline correction of pupil-size data}}.
\newblock {\emph{\JournalTitle{Behav. Res. Methods}}} \textbf{\bibinfo{volume}{50}}, \bibinfo{pages}{94--106}, \href{https://doi.org/10/ggxvtw}{10/ggxvtw} (\bibinfo{year}{2018}).

\bibitem{kundel1978visual}
\bibinfo{author}{Kundel, H.~L.}, \bibinfo{author}{Nodine, C.~F.} \& \bibinfo{author}{Carmody, D.}
\newblock \bibinfo{journal}{\bibinfo{title}{Visual scanning, pattern recognition and decision-making in pulmonary nodule detection}}.
\newblock {\emph{\JournalTitle{Invest. Radiol.}}} \textbf{\bibinfo{volume}{13}}, \bibinfo{pages}{175--181}, \href{https://doi.org/10/cgfqpn}{10/cgfqpn} (\bibinfo{year}{1978}).

\bibitem{hanby1992inter}
\bibinfo{author}{Hanby, A.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{An inter-observer and intra-observer variability study on the diagnosis of lymph node biopsy specimens}}.
\newblock {\emph{\JournalTitle{Eur. J. Cancer}}} \textbf{\bibinfo{volume}{28}}, \bibinfo{pages}{1858--1862}, \href{https://doi.org/10/ftrg6v}{10/ftrg6v} (\bibinfo{year}{1992}).

\bibitem{wilkinson2016fair}
\bibinfo{author}{Wilkinson, M.~D.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{{The FAIR Guiding Principles for scientific data management and stewardship}}}.
\newblock {\emph{\JournalTitle{Sci. Data.}}} \textbf{\bibinfo{volume}{3}}, \bibinfo{pages}{1--9}, \href{https://doi.org/10/bdd4}{10/bdd4} (\bibinfo{year}{2016}).

\bibitem{riggi2026lobular}
\bibinfo{author}{Riggi, J.~A.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Lobular cancerization in biopsy-diagnosed ductal carcinoma in situ (dcis) of the breast: a detailed histopathological evaluation and reproducibility study}}.
\newblock {\emph{\JournalTitle{DiagnPath}}} \href{https://doi.org/10/rvbm}{10/rvbm} (\bibinfo{year}{2026}).

\bibitem{abdel2022inter}
\bibinfo{author}{Abdel-Halim, C.~N.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Inter-and intrarater reliability and agreement among danish head and neck pathologists assessing extranodal extension in lymph node metastases from oropharyngeal squamous cell carcinomas}}.
\newblock {\emph{\JournalTitle{Head Neck Pathol.}}} \textbf{\bibinfo{volume}{16}}, \bibinfo{pages}{1082--1090}, \href{https://doi.org/10/rvbn}{10/rvbn} (\bibinfo{year}{2022}).

\bibitem{mandrekar2010receiver}
\bibinfo{author}{Mandrekar, J.~N.}
\newblock \bibinfo{journal}{\bibinfo{title}{Receiver operating characteristic curve in diagnostic test assessment}}.
\newblock {\emph{\JournalTitle{Journal of thoracic oncology}}} \textbf{\bibinfo{volume}{5}}, \bibinfo{pages}{1315--1316} (\bibinfo{year}{2010}).

\bibitem{landis1977measurement}
\bibinfo{author}{Landis, J.~R.} \& \bibinfo{author}{Koch, G.~G.}
\newblock \bibinfo{journal}{\bibinfo{title}{The measurement of observer agreement for categorical data}}.
\newblock {\emph{\JournalTitle{Biometrics}}} \textbf{\bibinfo{volume}{33}}, \bibinfo{pages}{159--174}, \href{https://doi.org/10.2307/2529310}{10.2307/2529310} (\bibinfo{year}{1977}).

\bibitem{simon1957models}
\bibinfo{author}{Herbert, S.~A.}
\newblock \emph{\bibinfo{title}{{Models of Man}}} (\bibinfo{publisher}{{John Wiley \& Sons, Inc.}}, \bibinfo{year}{1957}).

\bibitem{wolfe2022normal}
\bibinfo{author}{Wolfe, J.~M.}, \bibinfo{author}{Kosovicheva, A.} \& \bibinfo{author}{Wolfe, B.}
\newblock \bibinfo{journal}{\bibinfo{title}{Normal blindness: When we look but fail to see}}.
\newblock {\emph{\JournalTitle{Trends Cognit. Sci.}}} \textbf{\bibinfo{volume}{26}}, \bibinfo{pages}{809--819}, \href{https://doi.org/10/gtwm3x}{10/gtwm3x} (\bibinfo{year}{2022}).

\end{thebibliography}

